Approximate Range Emptiness in Constant Time and Optimal Space

This paper studies the \emph{$\varepsilon$-approximate range emptiness} problem, where the task is to represent a set $S$ of $n$ points from $\{0,\ldots,U-1\}$ and answer emptiness queries of the form "$[a ; b]\cap S \neq \emptyset$ ?" with a probability of \emph{false positives} allowed. This generalizes the functionality of \emph{Bloom filters} from single point queries to any interval length $L$. Setting the false positive rate to $\varepsilon/L$ and performing $L$ queries, Bloom filters yield a solution to this problem with space $O(n \lg(L/\varepsilon))$ bits, false positive probability bounded by $\varepsilon$ for intervals of length up to $L$, using query time $O(L \lg(L/\varepsilon))$. Our first contribution is to show that the space/error trade-off cannot be improved asymptotically: Any data structure for answering approximate range emptiness queries on intervals of length up to $L$ with false positive probability $\varepsilon$, must use space $\Omega(n \lg(L/\varepsilon)) - O(n)$ bits. On the positive side we show that the query time can be improved greatly, to constant time, while matching our space lower bound up to a lower order additive term. This result is achieved through a succinct data structure for (non-approximate 1d) range emptiness/reporting queries, which may be of independent interest.

==> squish-macros.tex <==
% !TEX root =  do-all.tex

%%%%%%%%%%%%%%%%%%%%  FOR COMMENTS  %%%%%%%%%%%%%%%%%%%%%%%

% allow toggle between full and short:

%\newcommand{\full}[1]{\#{\bf #1}\# }  %%leave for combined version
\newcommand{\full}[1]{}               %%leave for short version
%\newcommand{\full}[1]{#1}              %%leave for full version

%\newcommand{\short}[1]{\${\em #1}\$ } %%leave for combined version
\newcommand{\short}[1]{#1}            %%leave for short version
%\newcommand{\short}[1]{}               %%leave for full version

% named comments:
%\newcommand{\estie}[1]{\textbf{Estie:} #1}
%\newcommand{\michael}[1]{\textbf{Michael:} #1}
%\newcommand{\joe}[1]{\textbf{Joe:} #1}

% to blank out text:
\newcommand{\old}[1]{{}}

\newcommand{\comm}[1]{{\em COMMENT: #1}}

% margin comments:
% \newcommand{\comment}[1]{\marginpar{{\footnotesize #1}}}

%%%%%%%%%%%%%% SOME ABBREVIATIONS AND NOTATIONS %%%%%%%%%%%%%%

\newcommand{\eps}{\varepsilon}               % epsilon

\def\A{{\cal A}}
\def\B{{\cal B}}
\def\C{{\cal C}}
\def\D{{\cal D}}
\def\E{{\cal E}}
\def\F{{\cal F}}
\def\G{{\cal G}}
\def\H{{\cal H}}
\def\I{{\cal I}}
\def\J{{\cal J}}
\def\K{{\cal K}}
\def\L{{\cal L}}
\def\M{{\cal M}}
\def\N{{\cal N}}
\def\O{{\cal O}}
\def\P{{\cal P}}
\def\Q{{\cal Q}}
\def\R{{\cal R}}
\def\S{{\cal S}}
\def\T{{\cal T}}
\def\U{{\cal U}}
\def\V{{\cal V}}
\def\W{{\cal W}}
\def\X{{\cal X}}
\def\Y{{\cal Y}}
\def\Z{{\cal Z}}

%%%%%%%%%%%%%%%%%%%%%% SQUISHTEX  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Very flexible definitions of \section, \subsection, \subsubsection, and
% \paragraph.  The lengths \above[sub[sub]]sectionskip, \aboveparagraphskip,
% \below[sub[sub]]sectionskip, and \belowparagraphskip control the space around
% the headings.  If the below skips are negative, the section title is on the
% same line as the next paragraph.  The commands \[sub[sub]]sectionfont and
% \paragraphfont define the fonts for the headings.  By default, they produce
% the same effect as the article document class.
\newlength\abovesectionskip
\abovesectionskip=3.5ex plus .2ex minus 1ex
\newlength\belowsectionskip
\belowsectionskip=2.3ex plus .2ex
\def\sectionfont{\normalfont\Large\bfseries}
\newlength\abovesubsectionskip
\abovesubsectionskip=3.25ex plus .2ex minus 1ex
\newlength\belowsubsectionskip
\belowsubsectionskip=1.5ex plus .2ex
\def\subsectionfont{\normalfont\large\bfseries}
\newlength\abovesubsubsectionskip
\abovesubsubsectionskip=3.25ex plus .2ex minus 1ex
\newlength\belowsubsubsectionskip
\belowsubsubsectionskip=1.5ex plus .2ex
\def\subsubsectionfont{\normalfont\normalsize\bfseries}
\newlength\aboveparagraphskip
\aboveparagraphskip=-3.25ex plus 1ex minus .2ex
\newlength\belowparagraphskip
\belowparagraphskip=-1em
\def\paragraphfont{\normalfont\normalsize\bfseries}
\makeatletter
\def\section{\@startsection{section}{1}{\z@}{-\abovesectionskip}%
              {\belowsectionskip}{\sectionfont}}
\def\subsection{\@startsection{subsection}{1}{\z@}{-\abovesubsectionskip}%
                 {\belowsubsectionskip}{\subsectionfont}}
\def\subsubsection{\@startsection{subsubsection}{1}{\z@}%
                    {-\abovesubsubsectionskip}{\belowsubsubsectionskip}%
                    {\subsubsectionfont}}
\def\paragraph{\@startsection{paragraph}{4}{\z@}{-\aboveparagraphskip}%
                {\belowparagraphskip}{\paragraphfont}}
\makeatother

% Here are some good tight spacings for sections.
\abovesectionskip=1ex plus .5ex minus .5ex
\belowsectionskip=.5ex plus .5ex minus .25ex
\abovesubsectionskip=.75ex plus .75ex minus .375ex
%\abovesubsectionskip=.5ex plus .5ex minus .25ex
\belowsubsectionskip=.5ex plus .5ex minus .25ex
\aboveparagraphskip=.5ex plus .5ex minus .25ex
%\aboveparagraphskip=.25ex plus .25ex minus .125ex
\abovesubsubsectionskip=.5ex plus .5ex minus .25ex
\belowsubsubsectionskip=-1em

% Times font is thinner and saves space
\usepackage{times}

% Decrease space around theorems and such
\partopsep=3pt
\parsep=0pt
\topsep=0pt

% Reduce the extra space caused by displaymath (\[ ... \])
\abovedisplayskip=2pt plus 1pt minus 1pt
\belowdisplayskip=2pt plus 1pt minus 1pt
\abovedisplayshortskip=1pt plus 1pt minus 1pt
\belowdisplayshortskip=1pt plus 1pt minus 1pt

% Figure spacing
\abovecaptionskip=0pt           % space between figure and caption
\belowcaptionskip=0pt           % space after caption except for bottom figure
\intextsep=7pt plus 3pt        % space between [h]ere figure and text
\textfloatsep=7pt plus 3pt     % space between [t]op or [b]ottom figure & text

% Compact itemize and enumerate.  Note that they use the same counters and
% symbols as the usual itemize and enumerate environments.
\def\compactify{\itemsep=0pt \topsep=0pt \partopsep=0pt \parsep=0pt}
\let\latexusecounter=\usecounter
\newenvironment{CompactItemize}
 {\def\usecounter{\compactify\latexusecounter}
  \begin{itemize}}
 {\end{itemize}\let\usecounter=\latexusecounter}
\newenvironment{CompactEnumerate}
 {\def\usecounter{\compactify\latexusecounter}
  \begin{enumerate}}
 {\end{enumerate}\let\usecounter=\latexusecounter}


%%%%%%%%%%%%%%%%%%%%%%% END SQUISH



